Long time $H^1$-stability of fast L2-1$_\sigma$ method on general nonuniform meshes for subdiffusion equations

In this work, the global-in-time $H^1$-stability of a fast L2-1$_\sigma$ method on general nonuniform meshes is studied for subdiffusion equations, where the convolution kernel in the Caputo fractional derivative is approximated by sum of exponentials. Under some mild restrictions on time stepsize, a bilinear form associated with the fast L2-1$_\sigma$ formula is proved to be positive semidefinite for all time. As a consequence, the uniform global-in-time $H^1$-stability of the fast L2-1$_\sigma$ schemes can be derived for both linear and semilinear subdiffusion equations, in the sense that the $H^1$-norm is uniformly bounded as the time tends to infinity. To the best of our knowledge, this appears to be the first work for the global-in-time $H^1$-stability of fast L2-1$_\sigma$ scheme on general nonuniform meshes for subdiffusion equations. Moreover, the sharp finite time $H^1$-error estimate for the fast L2-1$_\sigma$ schemes is reproved based on more delicate analysis of coefficients where the restriction on time step ratios is relaxed comparing to existing works.

==> FastL2_1sigma(SOE)_nonuniform(quanwuyang) (Copy)/tmp_L2nonuniform_siam_header.tex <==
\title{$H^1$-stability of an L2-type method on general nonuniform meshes for subdiffusion equation\thanks{Submitted in June 2022.}}

\author{
Chaoyu Quan
\thanks{SUSTech International Center for Mathematics, Southern University of Science and Technology, Shenzhen, P.R. China (\email{quancy@sustech.edu.cn}).}
\and
Xu Wu
\thanks{Department of Mathematics,  Harbin Institute of Technology, Harbin 150001, China; Department of Mathematics, Southern University of Science and Technology, Shenzhen, China (\email{11849596@mail.sustech.edu.cn}).}
}


% Custom SIAM macro to insert headers
\headers{$H^1$-stability of L2-type method}{C. Quan and X. Wu}


==> FastL2_1sigma(SOE)_nonuniform(quanwuyang) (Copy)/tmp_SOE_L21sigma_header.tex <==
\title{Long time $H^1$-stability of fast L2-1$_\sigma$ method on general nonuniform meshes for subdiffusion equations\thanks{Submitted in Nov 2022.}}

\author{
Chaoyu Quan
\thanks{SUSTech International Center for Mathematics, Southern University of Science and Technology, Shenzhen, P.R. China (\email{quancy@sustech.edu.cn}).}
\and
Xu Wu
\thanks{Department of Mathematics,  Harbin Institute of Technology, Harbin 150001, China; Department of Mathematics, Southern University of Science and Technology, Shenzhen, China (\email{11849596@mail.sustech.edu.cn}).}
\and
Jiang Yang
\thanks{Department of Mathematics, SUSTech International Center for Mathematics \& National Center for Applied Mathematics Shenzhen (NCAMS), Guangdong Provincial Key Laboratory of Computational Science and Material Design, Southern University of Science and Technology, Shenzhen,China  (\email{yangj7@sustech.edu.cn}).}
}


% Custom SIAM macro to insert headers
\headers{Long time $H^1$-stability of fast L2-1$_\sigma$ method}{C. Quan, X. Wu and J. Yang}


==> tmp_L2nonuniform_siam_header.tex <==
\title{$H^1$-stability of an L2-type method on general nonuniform meshes for subdiffusion equation\thanks{Submitted in June 2022.}}

\author{
Chaoyu Quan
\thanks{SUSTech International Center for Mathematics, Southern University of Science and Technology, Shenzhen, P.R. China (\email{quancy@sustech.edu.cn}).}
\and
Xu Wu
\thanks{Department of Mathematics,  Harbin Institute of Technology, Harbin 150001, China; Department of Mathematics, Southern University of Science and Technology, Shenzhen, China (\email{11849596@mail.sustech.edu.cn}).}
}


% Custom SIAM macro to insert headers
\headers{$H^1$-stability of L2-type method}{C. Quan and X. Wu}

